Multivariate Quantum Signal Processing

We develop Multivariate Quantum Signal Processing for designing matrix-valued transformations of multiple noncommuting nonnormal block-encoded matrices. Our framework equips quantum transducers with the analytic structure of multiport Infinite-Impulse-Response (IIR) filters and establishes a transfer-function methodology for designing quantum query algorithms. Efficiently computable analytic bounds that hold uniformly across the oracle promise yield efficient quantum circuits with logarithmic error dependence and near-unity success probability, paralleling the approximation-theoretic guarantees of univariate QSP/QSVT. We provide a complete characterization of achievable transfer functions and a principled library of analytic IIR components. Our modular designs greatly improve or resolve the per-oracle query complexity of open multi-oracle problems: (1) Hamiltonian simulation under $H=\sum_j H_j$ with weighted quasinorm cost $\approx t\langle\vec\lambda,\vec C\rangle_{1/2}+\mathcal{O}(\|\vec C\|_1\log(1/\epsilon))$ for block-encoding normalizations $\vec\lambda$ and costs $\vec C$; (2) sparse simulation with optimal time--norm $\Theta(\sqrt{d}\|H\|_{\rm 1\to2}t)$ and additive error dependence; (3) solving linear systems and (4) differential equations under minimal matrix assumptions with optimal weighted state-preparation and multi-term cost; (5) ground-state preparation and energy estimation; (6) generalized eigenvalue problems. We apply these to exactly simulate downfolded Hamiltonians with leading cost $t\langle\vec\lambda_{\rm eff},\vec C_{\rm eff}\rangle_{1/2}$ further reduced by fractional dynamic correlation energy contributions from coarse-grained Hamiltonians, and show similar classical-data-input-reduction results for multiscale graph classification via Kron reduction. We also show the online generalization with anisotropic Kalman filtering of streaming quantum data.

==> libraries/IIR/examples/SelectedBlock.tex <==
% SelectedBlock.tex — A encoded operator is not the full unitary output
% Type: Finite circuit. Dependencies: none.
% Load iir-tikz.sty once. Import with \IIRDiagram{SelectedBlock}.
% Edit the named nodes and the explicit \draw lines below.
% Solid = public; dashed = private relative to this diagram's boundary.
\begin{tikzpicture}[iir]
%
\node[iir/gate] (unitary) at (0,0) {$U$};
%
\draw[iir/public] (-2.5,0) -- node[above] {$\IIRKet0_a\IIRKet\psi$} (unitary.west);
%
\draw[iir/public] (unitary.east) -- node[above] {$\IIRKet{\psi_{\rm out}}$} (2.5,0);
%
\node[iir/note] at (0,-.8) {$\IIRKet{\psi_{\rm out}}=\IIRKet0_a B\IIRKet\psi+\boldsymbol{r}$;\quad
%
$(\IIRBra0_a\otimes I_{\mathcal H})\boldsymbol{r}=0$.};
%
\end{tikzpicture}


==> libraries/IIR/unified-styles.tex <==
% Compatibility names inherit appearance from the existing IIR library.
\tikzset{
%
iir/quantum-control/.style={iir/public},
%
iir/coupling/.style={{Latex[length=1.6mm]}-{Latex[length=1.6mm]},line width=.6pt},
%
iir/axis/.style={-{Latex[length=1.6mm]},line width=.4pt},
%
qsys/.style={iir/box,minimum height=7mm}, qwire/.style={iir/public},
%
qfeedback/.style={iir/private}, qcoupling/.style={iir/coupling},
%
qlabel/.style={iir/note},
%
qlsp box/.style={iir/box,minimum height=6.5mm},
%
qlsp wire/.style={iir/public},qlsp private/.style={iir/private},
%
qlsp load/.style={iir/coupling},
%
gsp/.style={iir},gsp/box/.style={iir/box},gsp/system/.style={iir/system},
%
gsp/pub/.style={iir/public},gsp/priv/.style={iir/private},
%
gsp/control/.style={iir/quantum-control},gsp/note/.style={iir/note},
%
spbox/.style={iir/gate,minimum height=8mm,minimum width=22mm},
%
spwire/.style={iir/public},spfeedback/.style={iir/private},
%
splabel/.style={iir/note,fill=white,inner sep=1pt}
%
}
%
\providecommand{\GSPPorts}[1]{\IIRPorts{#1}}

